Practical Detectability for Persistent Lock-Free Data Structures

Persistent memory (PM) is an emerging class of storage technology that combines the benefits of DRAM and SSD. This characteristic inspires research on persistent objects in PM with fine-grained concurrency control. Among such objects, persistent lock-free data structures (DSs) are particularly interesting thanks to their efficiency and scalability. One of the most widely used correctness criteria for persistent lock-free DSs is durable linearizability (Izraelevitz et. al., DISC 2016). However, durable linearizability is insufficient to use persistent DSs for fault-tolerant systems requiring exactly-once semantics for storage systems, because we may not be able to detect whether an operation is performed when a crash occurs. We present a practical programming framework for persistent lock-free DSs with detectability. In contrast to the prior work on such DSs, our framework supports (1) primitive detectable operations such as space-efficient compare-and-swap, insertion, and deletion; (2) systematic transformation of lock-free DSs in DRAM into those in PM requiring modest efforts; (3) comparable performance with non-detectable DSs by DRAM scratchpad optimization; and (4) recovery from both full system and thread crashes. The key idea is memento objects serving as a lightweight, precise, and per-thread checkpoints in PM. As a case study, we implement lock-free and combining queues and hash tables with detectability that outperform (and perform comparably) the state-of-the-art DSs with (and without, respectively) detectability.

==> pgflibrarymykeys.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
%         rmem executable model                                      %
%                                                                    %
%   Shaked Flur, University of Cambridge                             %
%   Jon French, University of Cambridge                              %
%   Kathryn Gray, University of Cambridge (when this work was done)  %
%   Robert Norton-Wright, University of Cambridge                    %
%   Christopher Pulte, University of Cambridge                       %
%   Susmit Sarkar, University of St Andrews                          %
%   Peter Sewell, University of Cambridge                            %
%                                                                    %
%  This file is copyright 2010-2017 by the authors above.            %
%                                                                    %
%  All rights reserved.                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% This library should be loaded using '\usepgflibrary{mykeys}'

\pgfkeys{
  % #1 - package name
  % #2 - warning/error message
  % #3 - help message (as in "Type H <return> for immediate help")
  /utils/package warning/.code 2 args={\PackageWarning{#1}{#2}},
  /utils/package error/.code n args={3}{\PackageError{#1}{#2}{#3}},
}

\pgfkeys{
  % <key>/.get key parts=<macro>
  % Defines <macro> to be fully qualified <key>, '<macro>name' to be
  % the key name of <key> and '<macro>path' to be the path of <key>
  % (i.e. <macro>path/<macro>name = <macro>).
  % For example, after '\tikzset{foo/.get key parts=\mykey}' \mykey expands
  % to '/tikz/foo', \mykeyname expands to 'foo' and \mykeypath expands
  % to '/tikz'.
  /handlers/.get key parts/.code={%
    \edef#1{\pgfkeyscurrentpath}%
    \edef\pgfkeyscurrentkey{\pgfkeyscurrentpath}%
    \pgfkeyssplitpath{}%
    \count@\escapechar \escapechar\m@ne%
      \expandafter\edef\csname\string#1name\endcsname{\pgfkeyscurrentname}%
      \expandafter\edef\csname\string#1path\endcsname{\pgfkeyscurrentpath}%
    \escapechar\count@%
  }
}

\pgfkeys{
  % <path>/.cd scope={<key list>} evaluates <key list> with <path> as
  % default path.
  /handlers/.cd scope/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    /utils/exec={\expandafter\pgfqkeys\expandafter{\myk@key}{#1}},
  }
}

\pgfkeys{
  % <key>/.export to=<path> similar to <path>/<key-name>/.forward to=<key>
  /handlers/.export to/.style={
    \pgfkeyscurrentpath/.get key parts=\@myk@key,
    #1/\@myk@keyname/.estyle={\@myk@key={##1}},
  }
}

\pgfkeys{
  % <key>/.selected=<value> has the effect of <key>/\pgfkeysvalueof{<key>}=<value>
  % Example:
  %   foo/.initial=a,
  %   foo/.selected=hello, % => foo/a=hello
  %   foo=b,
  %   foo/.selected=world  % => foo/b=world
  /handlers/.selected/.style={
    \pgfkeyscurrentpath/\pgfkeysvalueof{\pgfkeyscurrentpath}={#1},
  }
}

\pgfkeys{
  % <key>/.try selected=<value> has the effect of <key>/\pgfkeysvalueof{<key>}/.try=<value>
  /handlers/.try selected/.style={
    \pgfkeyscurrentpath/\pgfkeysvalueof{\pgfkeyscurrentpath}/.try={#1},
  },
  % '<key>/.is choice with no match' is the same as '<key>/.is choice'
  % with the addition that if '<key>=<value>' is called and '<key>/<value>'
  % is not set, '<key>/.no match=<value>' is called.
  /handlers/.is choice with no match/.style={
    \pgfkeyscurrentpath/.get key parts=\@myk@key,
    \@myk@key/.is choice,
    \@myk@key/.unknown/.ecode={%
      \noexpand\let\noexpand\@unknown@name=\noexpand\pgfkeyscurrentname%
      \noexpand\pgfkeysalso{%
        \@myk@key/.no match/.expand once=\noexpand\@unknown@name,%
      }%
    },
  }
}

\long\def\myk@ifboolexpe#1 then #2 else #3\par{%
  \ifboolexpe{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}%
}
\long\def\myk@ifboolexpr#1 then #2 else #3\par{%
  \ifboolexpr{#1}{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}%
}

\def\myk@evaluateif#1 then #2 else #3\par{%
  \pgfmathparse{#1}%
  \ifdim\pgfmathresult pt=0pt\relax%
    \pgfkeysalso{#3}%
  \else%
    \pgfkeysalso{#2}%
  \fi%
}

\pgfkeys{
  % /utils/ifboolexpe={<expression>} then {<true key list>}[ else {<false key list>}]
  % Evaluates <expression> using \ifboolexpe and then <true key list>
  % or <false key list>, according to the result.
  /utils/ifboolexpe/.code args={#1 then #2#3}{%
    \ifstrempty{#3}{%
      \myk@ifboolexpe{#1} then {#2} else {}\par%
    }{% else
      \myk@ifboolexpe{#1} then {#2}#3\par%
    }%
  },
  /utils/ifboolexpr/.code args={#1 then #2#3}{%
    \ifstrempty{#3}{%
      \myk@ifboolexpr{#1} then {#2} else {}\par%
    }{% else
      \myk@ifboolexpr{#1} then {#2}#3\par%
    }%
  },
  % /tikz/evaluate if={<expression>} then {<true key list>}[ else {<false key list>}]
  % Evaluates <expression> using \pgfmathparse and then, if the result
  % is different than 0 executes <true key list>, otherwise executes
  % <false key list>.
  /tikz/evaluate if/.code args={#1 then #2#3}{%
    \ifstrempty{#3}{%
      \myk@evaluateif{#1} then {#2} else {}\par%
    }{% else
      \myk@evaluateif{#1} then {#2}#3\par%
    }%
  },
  % For any <key> that was set up as a flag:
  % '<key>/.if true=then {<true key list>}[ else {<false key list>}]'
  % '<key>/.if false=then {<true key list>}[ else {<false key list>}]'
  % evaluate <true key list> or <false key list> according to the flag
  % (i.e. <key>/.@boolexpe).
  /handlers/.if true/.code args={then #1#2}{%
    \edef\myk@key{\pgfkeyscurrentpath}%
    \pgfkeysifdefined{\myk@key/.@boolexpe}{%
      \pgfkeysgetvalue{\myk@key/.@boolexpe}{\myk@boolexpe}%
      \ifstrempty{#2}{%
        \expandafter\myk@ifboolexpe\expandafter{\myk@boolexpe} then {#1} else {}\par%
      }{% else
        \expandafter\myk@ifboolexpe\expandafter{\myk@boolexpe} then {#1}#2\par%
      }%
    }{% else
      \PackageError{pgflibrarymykeys}{'\myk@key' is not a boolean flag}{Did you forget '\myk@key/.is if flag=...'?}%
    }%
  },
  /handlers/.if false/.code args={then #1#2}{
    \edef\myk@key{\pgfkeyscurrentpath}%
    \pgfkeysifdefined{\myk@key/.@boolexpe}{%
      \pgfkeysgetvalue{\myk@key/.@boolexpe}{\myk@boolexpe}%
      \edef\myk@boolexpe{not (\expandonce\myk@boolexpe)}%
      \ifstrempty{#2}{%
        \expandafter\myk@ifboolexpe\expandafter{\myk@boolexpe} then {#1} else {}\par%
      }{% else
        \expandafter\myk@ifboolexpe\expandafter{\myk@boolexpe} then {#1}#2\par%
      }%
    }{% else
      \PackageError{pgflibrarymykeys}{'\myk@key' is not a boolean flag}{Did you forget '\myk@key/.is if flag=...'?}%
    }%
  },
  % <key>/.is flag=<true|false> (default true)
  % Sets up <key> for the '.if true' and '.if false' handlers.
  % <key> or <key>=true to set the flag to true, and <key>=false to set
  % it to false.
  /handlers/.is flag/.style={
    \pgfkeyscurrentpath/.get key parts=\@myk@key,
    \@myk@key/.@boolexpe/.initial=,
    \@myk@key/true/.estyle={\@myk@key/.@boolexpe={bool {true}}},
    \@myk@key/false/.estyle={\@myk@key/.@boolexpe={bool {false}}},
    \@myk@key/.is choice,
    \@myk@key/.default=true,
    \@myk@key={#1},
  },
  % <key>/.is if flag=<TeX-if name>
  % Similar to the PGF '.is if' but also sets up <key> as a flag.
  /handlers/.is if flag/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.@boolexpe/.initial={bool {#1}},
    \myk@key/.is if={#1},
  },
  % <key>/.is global if flag=<TeX-if name>
  % Similar to '.is if flag' but sets the 'if' globally.
  /handlers/.is global if flag/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.@boolexpe/.initial={bool {#1}},
    \myk@key/true/.code={\global\csname #1true\endcsname},
    \myk@key/false/.code={\global\csname #1false\endcsname},
    \myk@key/.no match/.estyle={
      /errors/boolean expected={\csname myk@key\endcsname}{##1},
    },
    \myk@key/.is choice with no match,
    \myk@key/.default=true,
  },
  % <key>/.is toggle flag=<etoolbox toggle name>
  % Similar to '.is if flag' for flags defined with the etoolbox \newtoggle.
  /handlers/.is toggle flag/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.is choice,
    \myk@key/.default=true,
    \myk@key/true/.code={\toggletrue{#1}},
    \myk@key/false/.code={\togglefalse{#1}},
    \myk@key/.@boolexpe/.initial={togl {#1}},
  },
  % <key>/.if defined=then {<true key list>}[ else {<false key list>}]
  % If <key> is defined evaluates <true key list>, otherwise evaluates <false key list>.
  /handlers/.if defined/.style args={then #1#2}{
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    /utils/ifboolexpe={test {\pgfkeysifdefined{\myk@key}}} then {#1}#2,
  },
  % <key>/.if defined value={<macro>} then {<true key list>}[ else {<false key list>}]
  % If <key> is defined, sets <macro> to the value of <key>
  % and evaluates <true key list>, otherwise evaluates <false key list>.
  /handlers/.if defined value/.style args={#1 then #2#3}{
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.if defined=then {\myk@key/.get=#1,#2}#3,
  },
  % /utils/if no value={<#n>} then {<true keys>}[ else {<false keys>}]
  % evaluates <true keys> if <#n> is \pgfkeysnovalue, otherwise
  % evaluates <false keys>.
  /utils/if no value/.style args={#1 then #2#3}{%
    /utils/exec={\def\myk@temp{#1}},
    /utils/ifboolexpe={test {\ifdefequal{\myk@temp}{\pgfkeysnovalue@text}}} then {#2}#3,
  },
}

\pgfkeys{
  % <key>/.try with warning=<value>
  % Similar to '.try', but when the try fails prints a warning.
  /handlers/.try with warning/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.try={#1},
    /utils/ifboolexpe={not bool {pgfkeyssuccess}} then {%
      /utils/package warning/.expanded={pgflibrarymykeys}{The key '\myk@key' does not exist},
    },
  },
}

\pgfkeys{
  % <key>/.get with default={<macro>}{<value>}
  % Similar to /.get, but if <key> is not defined assignes <value> to
  % <macro> using \def.
  /handlers/.get with default/.style 2 args={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.if defined=then {
      \myk@key/.get=#1,
    } else {
      /utils/exec={\def#1{#2}},
    },
  },
  % <key>/.value of=<another key>
  % Equivalent to writing '<key>=\pgfkeysvalueof{<another key>}'
  % which is somewhat like the '.link' handler, only for predefined keys.
  % NOTE: <another key> must be a fully qualified key name.
  /handlers/.value of/.style={\pgfkeyscurrentpath=\pgfkeysvalueof{#1}},
}

\pgfkeys{
  % <key>/.global store in=<macro>
  % Similar to '.store in', except that <macro> is defined globally.
  /handlers/.global store in/.style={
    \pgfkeyscurrentpath/.code={\gdef#1{##1}},
  }
}

\pgfkeys{
  % <key>/.list append={<value>}
  % <key>/.list prepend={<value>}
  % <key>/.list reverse
  % Assuming the value of <key> is a comma separated list, apply the
  % selected list operation to it.
  /handlers/.list append/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.get=\myk@temp@the@list,
    /utils/ifboolexpe={test {\ifdefempty{\myk@temp@the@list}}} then {
      \myk@key={#1}
    } else {
      \myk@key/.append={,#1}
    },
  },
  /handlers/.list prepend/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.get=\myk@temp@the@list,
    /utils/ifboolexpe={test {\ifdefempty{\myk@temp@the@list}}} then {
      \myk@key={#1}
    } else {
      \myk@key/.prefix={#1,}
    },
  },
  /handlers/.list reverse/.style={
    \pgfkeyscurrentpath/.get key parts=\myk@key,
    \myk@key/.get=\myk@temp@the@list,
    \myk@key=,
    \myk@key/.list prepend/.list/.expanded={\myk@temp@the@list},
  }
}


==> tikzlibrarylitmus.aarch64.tex <==
\litmusset{
  AArch64/.style={
    /litmus/listing options/.if defined=then {
      /litmus/listing options/.prefix={language=AArch64,}
    },
    /litmus/base language,
    % Generated in pp.ml (pp_brief_write_kind):
    /litmus/mem access/Wrel/.code={W\textsubscript{rel}},
    /litmus/mem access/Wexc/.code={W\textsubscript{exc}},
    /litmus/mem access/We-r/.code={W\textsubscript{e-r}},
    % Generated in pp.ml (pp_brief_read_kind):
    /litmus/mem access/Racq/.code={R\textsubscript{acq}},
    /litmus/mem access/Rwacq/.code={R\textsubscript{wacq}},
    /litmus/mem access/Rexc/.code={R\textsubscript{exc}},
    /litmus/mem access/Re-a/.code={R\textsubscript{e-a}},
    /litmus/mem access/Rnt/.code={R\textsubscript{nt}},
    /litmus/isb/.litmus relation=litmusIndigo,
    /litmus/ctrl+isb/.litmus relation=litmusIndigo,
    /litmus/dmb/.litmus relation=litmusDarkGreen,
    /litmus/dmb sy/.litmus relation=litmusDarkGreen,
    /litmus/dmb st/.litmus relation=litmusDarkGreen,
    /litmus/dmb ld/.litmus relation=litmusDarkGreen,
    /litmus/dsb/.litmus relation=litmusDarkGreen,
    /litmus/dsb sy/.litmus relation=litmusDarkGreen,
    /litmus/dsb st/.litmus relation=litmusDarkGreen,
    /litmus/dsb ld/.litmus relation=litmusDarkGreen,
    /litmus/.cd scope={
      every AArch64/.try,
    },
  },
}


==> tikzlibrarylitmus.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
%         rmem executable model                                      %
%                                                                    %
%   Shaked Flur, University of Cambridge                             %
%   Jon French, University of Cambridge                              %
%   Kathryn Gray, University of Cambridge (when this work was done)  %
%   Robert Norton-Wright, University of Cambridge                    %
%   Christopher Pulte, University of Cambridge                       %
%   Susmit Sarkar, University of St Andrews                          %
%   Peter Sewell, University of Cambridge                            %
%                                                                    %
%  This file is copyright 2010-2017 by the authors above.            %
%                                                                    %
%  All rights reserved.                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% This library should be loaded using '\usetikzlibrary{litmus}'
% See tikz_example/example.tex for details on how to use this library

%%% TODO:
% - Add @ to all the keys that should not be accessible to users.
% - Evaluating multiple styles in a ".cd scope" is not safe, as the
%   first style might change the default path.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\RequirePackage{etoolbox}

% Load pgf/tikz libraries
\usepgflibrary{mykeys}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}
\usetikzlibrary{chains}
\usetikzlibrary{scopes}
\usetikzlibrary{matrix}
\usetikzlibrary{fit}
\usetikzlibrary{backgrounds}
\usetikzlibrary{math}

% \lit@ifnodeexists{<name or alias>}{<true>}{<false>}
\newcommand{\lit@ifnodeexists}[1]{%
  \ifcsequal{pgf@sh@pi@#1}{pgfpictureid}%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfkeys{
  /litmus/.is family,
  %%% pgf BUG: when defining "<path>/.search also=..." and then calling
  %%% "\pgfkeys{<path>/<unknown key>}" the error message complains that
  %%% "/handlers/.unknown/.@cmd" does not exist, instead of complaining
  %%% about "<path>/<unknown key>", this makes debugging harder.
  /litmus/.search also={/tikz},
  %
  % This is a bit of a hack to allow un-prefixed /litmus keys when
  % /tikz is the default path.
  % NOTE: /tikz/.unknown/.@cmd calls '/errors/unknown key' after
  % trying everything and failing.
  /litmus/append to tikz path search/.style={
    % Setup things only if we have not already done it
    /errors/unknown key/original/.@cmd/.if defined=then {} else {
      % Save a copy of the original '/errors/unknown key'
      /utils/exec={%
        \pgfkeysgetvalue{/errors/unknown key/.@cmd}{\lit@temp@unknown}%
        \pgfkeyslet{/errors/unknown key/original/.@cmd}{\lit@temp@unknown}%
      },
      % Redefine '/errors/unknown key' to look in /litmus before failing
      /errors/unknown key/.style 2 args={
        % ##1 is the unknown key (fully qualified)
        % ##2 is the value passed to the key
        ##1/.get key parts=\lit@key,
        /utils/ifboolexpr={test {\ifdefstring{\lit@keypath}{/tikz}}} then {
          % /tikz/.unknown uses \pgfkeys (instead of \pgfkeysalso) to
          % call "/errors/unknown key" so we need to switch back to /tikz
          /tikz,
          /litmus/\lit@keyname/.try={##2},
          /errors/unknown key/original/.retry={##1}{##2},
        } else {
          /errors/unknown key/original={##1}{##2},
        },
      },
      % By forwarding the keys "/errors/unknown key/.code 2 args" and
      % "/errors/unknown key/.style 2 args" we make it harder for
      % someone to overwrite the code above (instead the saved copy
      % will be overwritten).
      /errors/unknown key/.code 2 args/.forward to=/errors/unknown key/original/.code 2 args,
      /errors/unknown key/.style 2 args/.forward to=/errors/unknown key/original/.style 2 args,
    },
  },
}
\def\litmusset{\pgfqkeys{/litmus}}

\def\assem{\verb}

% By default \assem is \verb which cannot be used in macro arguments.
% Whenever we need to pass \assem in an argument we pass this instead:
\def\lit@internal@assem#1{{\ttfamily #1}}

% \chaincount{<chain>} returns the number of nodes on the chain
\newcommand{\chaincount}[1]{\csuse{tikz@lib@chain@count@#1}}

\newif\iflit@assem\lit@assemtrue
\litmusset{is assem litmus/.is if flag=lit@assem}

\newif\iflit@events\lit@eventstrue
\litmusset{is events litmus/.is if flag=lit@events}

\newif\iflit@hide@line\lit@hide@linefalse
\litmusset{hide line/.is global if flag=lit@hide@line}

\newif\iflit@needs@end@row\lit@needs@end@rowfalse

\newcounter{lit@ioid@sub}

\newif\iflit@last@inst\lit@last@instfalse

\def\lit@add@row@after#1#2{%
  % #1 - ioid of the instruction above
  % #2 - node text
  \iflit@assem%
    \lit@matrixendrow%
    \stepcounter{lit@ioid@sub}%
    \node[/litmus/assem/.expanded={#1-\arabic{lit@ioid@sub}}] {#2};%
  \fi%
}

% This is the end-of-row macro for 'instructions' matrix.
\def\litmusendinst{\futurelet\lit@tok\lit@endinst}
\def\lit@endinst{%
  \ifx\lit@tok\egroup%
    \global\lit@last@insttrue%
  \else%
    \global\lit@last@instfalse%
  \fi%
  \iflit@assem%
    \iflit@hide@line%
      \iflit@last@inst%
        \PackageWarning{litmus-tikz-library}{last line can not be completely hidden (\lit@ioid)}%
      \fi%
    \else%
      \pgfkeysifdefined{/tikz/pics/\lit@ioid/.@cmd}{%
        \iflit@events%
          \pgfmatrixnextcell%
          \pic {\lit@ioid};%
        \fi%
      }{}%
      % add rows as requested
      \pgfkeysifdefined{/litmus/assem \lit@ioid/insert rows after/.@cmd}{%
        \setcounter{lit@ioid@sub}{0}%
        \litmusset{assem \lit@ioid/insert rows after}%
      }{}%
      \iflit@last@inst\else%
        \lit@matrixendrow%
      \fi%
    \fi%
  \else%
    \pgfkeysifdefined{/tikz/pics/\lit@ioid/.@cmd}{%
      % The matrix must end with \pgfmatrixendrow (the one at the end
      % of this macro) so we have to do all the other \pgfmatrixendrow
      % just before the \pic, except, of course, for the very first \pic
      \iflit@needs@end@row%
        \lit@matrixendrow%
      \fi%
      \lit@needs@end@rowtrue%
      \pic {\lit@ioid};%
    }{}%
  \fi%
  \iflit@last@inst%
    \expandafter\lit@matrixendrow%
  \fi%
}

\def\lit@matrixendrow{\expandafter\pgfmatrixendrow\expandafter[\lit@add@space@after@row]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% typeset memory footprint

\newif\iflit@mixed@size\lit@mixed@sizetrue
\litmusset{is mixed-size/.is if flag=lit@mixed@size}

\litmusset{
  non-mixed-size/.style={
    /litmus/memfp/.code n args={4}{%
      \tikzmath{
        let \addr = ##1;
        let \offs = ##2;
        let \size = ##3;
        if \offs==0 then { print{\addr}; }
        else { print{\addr+\offs}; };
      }=##4%
    },
    /litmus/memrf/.code 2 args=rf,
    /litmus/memfr/.code 2 args=fr,
    /litmus/is mixed-size=false,
  },
}

\litmusset{
  old-mixed-size/memslices/.code 2 args={%
    \def\slices@temp{\@gobble}%
    \foreach \i/\j in {#2} {%
      \tikzmath{\size = int(\j - \i + 1);}%
      \ifnum\i=\z@%
        \xdef\slices@temp{\slices@temp,#1/\size}%
      \else%
        \xdef\slices@temp{\slices@temp,#1+\i/\size}%
      \fi%
    }%
    \slices@temp%
  },
  old-mixed-size/.style={
    /litmus/memfp/.code n args={4}{%
      \tikzmath{
        let \addr = ##1;
        let \offs = ##2;
        let \size = ##3;
        if \offs==0 then { print{\addr/\size}; }
        else { print{\addr+\offs/\size}; };
      }=##4%
    },
    /litmus/memrf/.code 2 args={rf\,\pgfkeysalso{/litmus/old-mixed-size/memslices={##1}{##2}}},
    /litmus/memfr/.code 2 args={fr\,\pgfkeysalso{/litmus/old-mixed-size/memslices={##1}{##2}}},
    /litmus/is mixed-size=true,
  },
}

\def\ifhex#1{\ifstrempty{#1}{\@secondoftwo}{\@ifhex-#1-0x\lit@del}}
\def\@ifhex#1-0x#2\lit@del{\ifstrempty{#1}}
\def\@gobblehex 0x#1\lit@del{#1}

\def\ifzero#1{\ifstrempty{#1}{\@secondoftwo}{\@ifzero-#1-0\lit@del}}
\def\@ifzero#1-0#2\lit@del{\ifstrempty{#1}}
\def\@gobblezeros #1\lit@del{\ifzero{#1}{\expandafter\@gobblezeros\@gobblezero #1\lit@del\lit@del}{#1}}
\def\@gobblezero 0#1\lit@del{#1}

\litmusset{
  symbol footprint/.code args={#1 from #2 to #3}{%
    \tikzmath{
      \litsymstart{#1} = #2;
      \litsymend{#1} = #3;
    }%
    \csdef{lit@sym@fp:#1}{exists}%
  },
  mixed-size/memslices/.code 2 args={%
    \def\slices@temp{\@gobble}%
    \foreach \i/\j in {#2} {%
      \ifx\i\j%
        \xdef\slices@temp{\slices@temp,\i}%
      \else%
        \xdef\slices@temp{\slices@temp,\i..\j}%
      \fi%
    }%
    #1[\slices@temp]%
  },
  event equal/.code={=},
  mixed-size/.style={
    /litmus/memfp/.code n args={4}{%
      \tikzmath{
        let \addr = ##1;
        let \offs = ##2;
        let \size = ##3;
        \i = int(\offs + \size - 1);
        if \size == 1 then { print{\addr[\offs]}; }
        else { print{\addr[\offs..\i]}; };
        print{\litmusset{event equal}};
        let \cond = \ifhex{##4}{1}{0};
        if \cond then {
          let \cond = \ifcsdef{lit@sym@fp:##1}{1}{0};
          if \cond then {
            print{0x};
            let \addrstart = \litsymstart{##1};
            let \addrend = \litsymend{##1};
            if \offs + \size <= \addrend then {
              for \i in {\offs + \size,...,\addrend}{
                print{\_\_};
              };
            };
            print{\@gobblehex##4\lit@del};
            if \addrstart + 1 <= \offs then {
              for \i in {\addrstart + 1,...,\offs}{
                print{\_\_};
              };
            };
          } else {
            print{%
              \edef\lit@val{\@gobblehex##4\lit@del}%
              \edef\lit@val{\expandafter\@gobblezeros\lit@val\lit@del}%
              \edef\lit@val{\expandafter\ifstrempty\expandafter{\lit@val}{0}{\lit@val}}%
              \pgfmathbasetodec{\lit@val}{\lit@val}{16}%
              \lit@val%
            };
          };
        } else {
          print{##4};
        };
      }%
    },
    /litmus/memrf/.code 2 args={rf\,\pgfkeysalso{/litmus/mixed-size/memslices={##1}{##2}}},
    /litmus/memfr/.code 2 args={fr\,\pgfkeysalso{/litmus/mixed-size/memslices={##1}{##2}}},
    /litmus/is mixed-size=true,
  },
}

\litmusset{non-mixed-size}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcount\maxassemlines

\newcommand{\lit@check@exists}{%
  {%
    \def\lit@check@exists@do##1{%
      \ifinlist{##1}{\lit@exists@list}{}{% else
        \PackageError{litmus-tikz-library}{event '##1' which you tried to change does not exist}{}%
      }%
    }%
    \forlistloop{\lit@check@exists@do}{\lit@check@exists@list}%
  }%
}

\litmusset{
  litmus arrow/.tip={Stealth[length=0.5em,inset=0.1em]},
  litmus internal/.style={
    /utils/exec={\global\maxassemlines=0},
    % If the assem/event 'text height' of the first instructions are
    % not identical the thread headers will not be aligned
    /tikz/start chain=threads going {/tikz/right=of \tikzchainprevious.north east, /tikz/matrix anchor=north west},
    /tikz/>=litmus arrow,
    /utils/exec={
      \gdef\lit@exists@list{}
      \gdef\lit@check@exists@list{}
    },
    /tikz/execute at end scope=\lit@check@exists,
  },
  kind/.is choice,
  kind/.default=full,
  kind/full/.style={
    /litmus/is assem litmus=true,
    /litmus/is events litmus=true,
    /litmus/simple instructions/.style={/litmus/@simple full},
    /litmus/litmus internal,
    /litmus/threads distance/.initial=6em,
    /litmus/header to instructions distance/.initial=0pt,
    /litmus/draw thread header/.style=,
    /litmus/disable edge routing,
    /litmus/.cd scope={
      every litmus/.try,
      every full litmus/.try,
    },
  },
  kind/assem/.style={
    /litmus/is assem litmus=true,
    /litmus/is events litmus=false,
    /litmus/simple instructions/.style={/litmus/@simple assem},
    /litmus/litmus internal,
    /litmus/threads distance/.initial=0pt,
    /litmus/header to instructions distance/.initial=0pt,
    /litmus/draw thread header/.style=,
    /litmus/disable edge routing,
    /litmus/.cd scope={
      every litmus/.try,
      every assem litmus/.try,
    },
%     /litmus/event/.append style=/litmus/hide,
%     /litmus/events box/.style=/litmus/hide,
    /litmus/instruction relations/.style=/litmus/hide,
    /litmus/event relations/.style=/litmus/hide,
  },
  kind/events/.style={
    /litmus/is assem litmus=false,
    /litmus/is events litmus=true,
    /litmus/simple instructions/.style={/litmus/@simple events},
    /litmus/litmus internal,
    /litmus/threads distance/.initial=3em,
    /litmus/header to instructions distance/.initial=0.5ex,
    /litmus/draw thread header/.style={/tikz/rectangle, /tikz/draw},
    /litmus/enable edge routing,
    /litmus/.cd scope={
      every litmus/.try,
      every events litmus/.try,
    },
    /litmus/code label position=none, % don't show code labels...
    % ...and change the key so it cannot be changed (e.g. by 'every litmus')
    /litmus/code label position/.code=,
    /litmus/assem internal/.append style=/litmus/hide,
  },
}

% This is a hack for .ps as it does not support opacity:
\@ifclasswith{standalone}{dvips}{
  \litmusset{
    kind/events/.append style={
      /litmus/assem internal/.append style={/tikz/scale=0.001, /tikz/transform shape},
    },
  }
}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzset{
  % The alias key does not work on matrices, that breaks 'on chain',
  % we fix it by adding another node with the expected name
  matrix on chain/.style={
    /tikz/matrix,
    /tikz/on chain={#1},
    % We forward all the alias arguments to 'matrix alias' and use it
    % to collect the aliases in \lit@alias@temp (csv)
    /utils/exec={\def\lit@alias@temp{\@gobble}},
    /temp/matrix alias/.code={\xdef\lit@alias@temp{\lit@alias@temp,##1}},
    /tikz/alias/.forward to=/temp/matrix alias,
    % We do not want to collect aliases in the cells
    /tikz/execute at begin cell={\pgfkeys{/temp/matrix alias/.code={}}},
    % Add to the end of the path a new simple node with all the aliases
    /tikz/append after command={
      node[fit=(\tikzlastnode),
        minimum size=0, inner sep=0, outer sep=0,
        alias/.list/.expand once=\lit@alias@temp,
      ] {}
    },
  },
}

% Hold the typical height and depth of assem text
\newlength{\assemheight}
\newlength{\assemdepth}

\litmusset{
  add thread header/.is flag=false,
  thread/.style={
    /litmus/thread id/.store in=\lit@tid,
    /litmus/thread id={#1},
    /litmus/add thread header,
    /litmus/.cd scope={
      every thread/.try=#1,
      thread #1/.try,
    },
  },
  thread header text/.store in=\lit@thread@header@text,
  thread header text={Thread~\lit@tid},
  thread header/.style={
    /tikz/alias/.expanded={thread \lit@tid\space header},
    /litmus/draw thread header/.try,
    /tikz/node distance/.value of=/litmus/header to instructions distance,
    /litmus/.cd scope={
      every thread header/.try/.expand once=\lit@tid,
      thread \lit@tid\space header/.try,
    },
  },
  ioid/.global store in=\lit@ioid,
  the code label/.global store in=\lit@code@label,
  instructions/.style={
    /utils/if no value={#1} then {} else {
      % There is no thread scope, but we still need to set \lit@tid.
      % We use global because '/tikz/append after command' is executed
      % in a different group.
      /litmus/thread id/.global store in=\lit@tid,
      /litmus/thread id={#1},
    },
    /litmus/the code label=,
    % 'node distance' must be set before 'on chain'
    /tikz/node distance/.value of=/litmus/threads distance,
    /tikz/matrix on chain=threads,
    /tikz/column sep=0.5em,
    /utils/exec={
      % Set \assemheight and \assemdepth to reasonable values
      \settoheight{\assemheight}{\pgfinterruptpicture\lit@internal@assem{X[/}\endpgfinterruptpicture}
      \global\assemheight=\assemheight
      \settodepth{\assemdepth}{\pgfinterruptpicture\lit@internal@assem{gjpqyQ[,/}\endpgfinterruptpicture}
      \global\assemdepth=\assemdepth
    },
    /litmus/is assem litmus/.if true=then {
      /litmus/is events litmus/.if true=then {
        /tikz/row sep={3ex,between origins}
      } else {
        /tikz/row sep={\assemheight+\assemdepth+1pt,between origins}
      }
    } else {
      /tikz/row sep={7ex,between origins}
    },
    /tikz/inner sep=0,
    /tikz/outer sep=0,
    /litmus/.cd scope={
      every instructions/.try,
    },
    /utils/exec={
      % Set \assemrowsep to the 'row sep' length part:
      \begingroup
        \def\@tempA##1,##2\par{##1}
        \edef\@tempB{\pgfmatrixrowsep}
        \edef\@tempC{\endgroup\noexpand\xdef\noexpand\assemrowsep{\expandafter\@tempA\@tempB,\par}}
      \@tempC
    },
    /litmus/add space after row/.store in=\lit@add@space@after@row,
    /litmus/add space after row=0pt,
    /tikz/execute at end matrix={%
      \ifnum\pgfmatrixcurrentrow>\maxassemlines\relax%
        \global\maxassemlines=\pgfmatrixcurrentrow%
      \fi%
    },
    /litmus/add thread header/.if true=then {
      /tikz/append after command={
        node[%
          % We check if \tikz@node@at has changed (becuase of user defined
          % styles), and if it has not, we set it to be above the instructions
          /utils/exec={\let\lit@temp@node@at=\tikz@node@at},
          /litmus/thread header,
          /utils/ifboolexpr={%
            test {\ifdefequal{\tikz@node@at}{\lit@temp@node@at}}%
          } then {above=of \tikzlastnode},
        ] {\lit@thread@header@text}%
      },
    },
  },
}

\newif\iflit@simple@endcell\lit@simple@endcelltrue
\def\lit@simple@event@endcell{\iflit@simple@endcell\egroup;\fi}

\def\lit@simple@cell#1{%
  \@ifnextchar !{%
    \lit@simple@endcellfalse\@gobble%
  }{% else
    \lit@simple@endcelltrue #1%
  }%
}
\def\lit@simple@event#1:{%
  \node[/litmus/.cd scope={event={#1}}] \bgroup%
    % when using "text width" tikz wraps the node text with a minipage that
    % redefines \\, we redefine it again so that "/tikz/execute at end cell"
    % can run as expected
    \let\\=\pgfmatrixendrow%
}


\def\lit@simple@assem{%
  \node[/litmus/assem] \bgroup%
    % when using "text width" tikz wraps the node text with a minipage that
    % redefines \\, we redefine it again so that "/tikz/execute at end cell"
    % can run as expected
    \let\\=\pgfmatrixendrow%
    \assem%
}

% a few wrappers of 'instructions' that make it easier to type simple tests
\litmusset{
  events column/.style={ % e.g.: a:R x=0
    /tikz/execute at begin cell={\lit@simple@cell\lit@simple@event},
    /tikz/execute at end cell={\expandafter\lit@simple@event@endcell},
  },
  assem column/.style={ % e.g.: |LDR W1,[X2]|
    /tikz/execute at begin cell={\lit@simple@cell\lit@simple@assem},
    /tikz/execute at end cell={\expandafter\lit@simple@event@endcell},
  },
  @simple instructions/.style={
    /litmus/add thread header,
    /litmus/instructions/.expanded=\chaincount{threads},
    /litmus/.cd scope={
      every simple instructions/.try,
    },
  },
  @simple events/.style={
    /litmus/@simple instructions,
    /tikz/column 1/.style=/litmus/events column,
    /litmus/.cd scope={
      every simple events/.try,
    },
  },
  @simple assem/.style={
    /litmus/@simple instructions,
    /tikz/column 1/.style=/litmus/assem column,
    /litmus/.cd scope={
      every simple assem/.try,
    },
  },
  @simple full/.style={
    /litmus/@simple instructions,
    /tikz/column 1/.style=/litmus/assem column,
    /tikz/column 2/.style=/litmus/events column,
    /litmus/.cd scope={
      every simple full/.try,
    },
  },
}

\newcommand{\lit@auxout@comtextwidth}[2]{%
  \immediate\write\@auxout{\string\lit@load@width{#1}{#2}}
}

\newcommand{\lit@load@width}[2]{%
  \csgdef{#1@litmusinstructionswidths}{#2}%
  \foreach \w [count=\t from 0] in {#2}{%
    \csxdef{#1@litmusinstructionswidth@\t}{\w}%
  }%
}

\pgfmathdeclarefunction{computedwidthofthread}{2}{%
  \begingroup%
    \ifcsdef{#1@litmusinstructionswidth@#2}{%
      \edef\res{\csuse{#1@litmusinstructionswidth@#2}}%
      \expandafter\pgf@x\res\relax%
    }{% else
      %%% NOTE: ^^J is a line-break, litmus.mk is looking for '^run latex again.'
      \PackageWarning{litmus-tikz-library}{Computed assem width of #1 is not available,^^Jrun latex again.}%
      \pgf@x0pt\relax%
    }%
    \pgfmathreturn\pgf@x%
  \endgroup%
}
\pgfkeys{
  /pgf/declare function={
    computedwidthof(\@uid)=computedwidthofthread("\@uid",\lit@tid);
  },
}

\colorlet{code label color}{black!50}

\litmusset{
  add row after/.style 2 args={%
    /litmus/assem #1/insert rows after/.append code={\lit@add@row@after{#1}{#2}}%
  },
  collect eiids/.style={ % #1 - an ioid
    /litmus/#1/eiids/.if defined value={\lit@eiids} then {
      % Barriers have no \pic but we still want an eiid comment
      /litmus/assem #1/eiids/.initial/.expanded=\lit@eiids,
    } else {
      /tikz/#1/eiids/.if defined value={\lit@eiids} then {
        /litmus/assem #1/eiids/.initial/.expanded=\lit@eiids,
      } else {
        /tikz/pics/#1-eiids/.@cmd/.if defined=then {
          /utils/exec={
            % Create the ioid's \pic without drawing it, to get the list
            % of eiids (placed in \lit@eiids).
            \begingroup
              \pgfpositionnodelater{\empty} % When a node is created, it is not
                                            % inserted into the current picture.
                                            % see 101.2.3 Deferred Node Positioning
              \pic {#1-eiids};
            \endgroup
          },
          /litmus/assem #1/eiids/.initial/.expand once=\lit@eiids,
        },
      },
    },
  },
  compute assem text width/.value required,
  compute assem text width/.style={
    % #1: some unique identifier; Used internally to store the widths.
    %     The pgf math function 'computedwidthof("#1")' expands to the
    %     computed widths of this diagram.
    /utils/ifboolexpe={test {\ifcsdef{#1@litmusinstructionswidths@uid}}} then {
      /utils/package warning={litmus-tikz-library}{'compute assem text width' expects a unique identifier, '#1' is already used.},
    } else {
      /utils/exec={\csgdef{#1@litmusinstructionswidths@uid}{true}},
      /utils/ifboolexpe={not test {\ifcsdef{#1@litmusinstructionswidths}}} then {
        % Width has not been computed in a previous run, compute it now
        % and save to the .aux file
        %%% NOTE: ^^J is a line-break, litmus.mk is looking for '^run latex again.'
        /utils/package warning={litmus-tikz-library}{Computing width of assem (#1),^^Jrun latex again.},
        /litmus/computed text width/.style={
          /tikz/text width=,
          /tikz/minimum size=0,
          /tikz/inner sep=0,
          /tikz/outer sep=0,
          /tikz/draw=none,
        },
        /tikz/execute at end scope={
          \def\lit@temp@widths{\@gobble}
          \tikzmath{
            int \t;
            coordinate \d;
            for \t in {1,...,int(\chaincount{threads})}{
              \d = (threads-\t.east)-(threads-\t.west);
              print{\xdef\lit@temp@widths{\lit@temp@widths,\dx}};
            };
          }
          \lit@auxout@comtextwidth{#1}{\lit@temp@widths}
        },
      },
    },
    % The following is outside the else because if the figure appears more than
    % once maybe we should use the same width (e.g. multiple slides in beamer)
    /pgf/declare function={
      computedwidth()=computedwidthof("#1");
    },
    /utils/ifboolexpe={test {\ifcsdef{#1@litmusinstructionswidths}}} then {
      % Width has been previously computed, saved to the .aux file and
      % loaded. Set 'text width' if it has not been set manually.
      /utils/exec={\lit@auxout@comtextwidth{#1}{\csuse{#1@litmusinstructionswidths}}},
      /litmus/computed text width/.style={
        /utils/ifboolexpe={test {\ifdefempty{\tikz@text@width}}} then {
          /tikz/text width=computedwidth,
        },
      },
    },
  },
  assem internal/.style={
    % #1 - ioid
    /tikz/name=assem #1,
    /litmus/ioid={#1},
    /litmus/hide line=false,
    /tikz/anchor=base west,
    % This makes assem rows consistent (i.e. rows of different threads align with each other)
    /tikz/text depth=\assemdepth,
    /tikz/text height=\assemrowsep - \assemdepth,
    /litmus/.cd scope={
      every assem/.try={\lit@code@label}{#1},
      assem #1/.try={\lit@code@label}{#1},
    },
    % 'execute at begin/end node' are accumelating so these have to be
    % after the user styles so the user's code is in the real begining
    % and user's end is before the eiids comment.
    /tikz/execute at begin node={
      \litmusset{inline code label/.selected/.expanded={\lit@code@label}{#1}}
    },
    /tikz/execute at end node={
      \litmusset{show eiids comment/.selected={#1}}
    },
    /litmus/computed text width/.try,
  },
  % 0-0 is a dummy ioid for hand written tests
  assem/.default=0-0,
  assem/.style={
    % #1 - ioid
    /litmus/collect eiids={#1},
    /litmus/assem internal={#1},
    % We always draw the edges, even when the events are not drawn,
    % hence, we add aliases to the assem so it can take the events place.
    /litmus/is events litmus/.if false=then {
      /litmus/assem #1/eiids/.if defined value={\lit@eiids@temp} then {
        /tikz/alias={#1},
        /tikz/alias/.list/.expand once=\lit@eiids@temp,
      },
    },
    /tikz/execute at end node={\gdef\lit@code@label{}},
  },
}

\litmusset{
  code label/.code 2 args={%
    % #1 - location label
    % #2 - ioid
    \ifstrempty{#1}{}{% else
      {\color{code label color}\lit@internal@assem{#1:}}%
    }%
  },
  inline code label/.initial=none,
  inline code label/inline/.style 2 args={/litmus/.cd scope={code label={#1}{#2}}},
  inline code label/left/.code 2 args={\llap{\litmusset{code label={#1}{#2}}}},
  inline code label/none/.style 2 args=,
  code label position/.is choice,
  code label position/above/.style={
    /litmus/assem label/.style={
      /litmus/the code label={##1},
      /tikz/node contents={%
        \litmusset{code label/.expanded={\lit@code@label}{\lit@tid-##1}}%
      },
      /litmus/assem internal/.expanded={\lit@tid-##1},
      /litmus/.cd scope={
        every assem label/.try,
      },
    },
    /litmus/inline code label=none,
  },
  code label position/inline/.style={
    /litmus/assem label/.style={
      /litmus/the code label={##1},
      /tikz/node contents=,
      /litmus/hide,
      /litmus/hide line,
    },
    /litmus/inline code label=inline,
  },
  code label position/left/.style={
    /litmus/assem label/.style={
      /litmus/the code label={##1},
      /tikz/node contents=,
      /litmus/hide,
      /litmus/hide line,
    },
    /litmus/inline code label=left,
  },
  code label position/none/.style={
    /litmus/assem label/.style={
      /litmus/ioid={##1},
      /litmus/the code label={##1},
      /tikz/node contents=,
      /litmus/hide,
      /litmus/hide line,
    },
    /litmus/inline code label=none,
  },
  code label position=above,
  eiids comment/.code={%
    \hfill{\color{red!60}\lit@internal@assem{//#1}}%
  },
  show eiids comment/.initial={\iflit@events false\else true\fi},
  show eiids comment/.default=true,
  show eiids comment/true/.style={
    /litmus/assem #1/eiids/.if defined value={\lit@eiids@temp} then {
      /litmus/.cd scope={
        eiids comment #1/.try/.expanded=\lit@eiids@temp,
        eiids comment/.retry/.expanded=\lit@eiids@temp,
      },
    },
  },
  show eiids comment/false/.style={},
}

\pgfkeys{
  /handlers/.mem read/.style={
    \pgfkeyscurrentpath/.get key parts=\lit@key,
    /litmus/\lit@keyname/.style/.expanded={/litmus/mem event={\lit@keyname:#1}},
    /litmus/eiids order/.list append/.expand once=\lit@keyname,
  },
  /handlers/.mem write/.style={
    \pgfkeyscurrentpath/.get key parts=\lit@key,
    /litmus/\lit@keyname/.style/.expanded={/litmus/mem event={\lit@keyname:#1}},
    /litmus/eiids order/.list append/.expand once=\lit@keyname,
  },
  /handlers/.events/.style={
    \pgfkeyscurrentpath/.get key parts=\lit@key,
    /tikz/\lit@keyname/.pic/.expanded={
      \noexpand\path[pic actions]
                    { [ /litmus/eiids order/.initial=,
                        /litmus/.cd scope={#1},
                        /litmus/events={\lit@keyname},
                        /litmus/eiids order/.get=\noexpand\lit@temp@eiids,
                        /litmus/event nodes/.initial=,
                        /litmus/add event node/.style={/litmus/event nodes/.append={node[/litmus/########1]}},
                        /litmus/add event node/.list/.expanded=\noexpand\lit@temp@eiids,
                      ]
                      \noexpand\pgfkeysvalueof{/litmus/event nodes}
                    }
                    node[/litmus/events box={\lit@keyname}] (\lit@keyname) {};
    },
    % The following .pic is used when we collect the eiids, it is not
    % used to draw anything.
    /tikz/\lit@keyname-eiids/.pic/.expanded={
      \noexpand\path
          { [ /litmus/eiids order/.initial=,
              /litmus/#1,
              /litmus/events={\lit@keyname},
              /litmus/eiids order/.get=\noexpand\lit@temp@eiids,
              /utils/exec={\noexpand\xdef\noexpand\lit@eiids{\noexpand\lit@temp@eiids}},
            ]
          } ;
    },
  },
}

\litmusset{
  events/.value required, % ioid
  events/.style={
    /tikz/local bounding box=lbbox,
    /tikz/node distance=1pt,
    /tikz/start chain=events going {/tikz/below=of \tikzchainprevious.south west, /tikz/anchor=north west},
    /litmus/event/.append style={/tikz/on chain=events},
    /litmus/.cd scope={
      every events/.try={#1},
      events #1/.try
    },
  },
  events box internal/.style={/tikz/inner sep=0},
  events box/.value required, % ioid
  events box/.style={
    /utils/exec={%
      \csxdef{lit@#1@tid}{\lit@tid}%
      \csxdef{lit@#1@row}{\the\pgfmatrixcurrentrow}%
    },
    /tikz/behind path,
    /tikz/fit=(lbbox),
    /litmus/events box internal,
    /litmus/.cd scope={
      every events box/.try={#1},
      events box #1/.try,
    },
  },
  show event label/.is flag=true,
  event label/.code={{\color{darkgray}#1:}},
  event/.value required,% eiid
  event/.style={
    % 'on chain=events' is added by 'events' so that 'event' can also
    % be used not on the chain (e.g. hand written diagrams).
    /tikz/name={#1-text},
    /utils/exec={%
      \csxdef{lit@#1@tid}{\lit@tid}%
      \csxdef{lit@#1@row}{\the\pgfmatrixcurrentrow}%
    },
    /tikz/node font=\sffamily,
    % If the heights of the first event in each thread do not match the
    % thread headers will not be aligned.
    /tikz/text height={height("abcdefghijklmnopqrstuvwxyz ABCDEFGHIJKLMNOPQRSTUVWXYZ 0123456789 =:/[]")},
    /litmus/.cd scope={
      every event/.try={#1},
      event #1/.try,
    },
    /litmus/show event label/.if true=then {
      /tikz/append after command={
        node[%
          anchor=base east,
          align=right,
          /litmus/.cd scope={
            every event label/.try={#1},
            event label #1/.try,
          },
        ] (#1-label) at (#1-text.base west) {\litmusset{event #1/eiid/.get with default={\lit@eiid}{#1}, event label/.expand once=\lit@eiid}}
        node[%
          fit={(#1-label)(#1-text)},
          inner sep=2pt,
          /litmus/.cd scope={
            every event box/.try={#1},
            event box #1/.try,
          },
        ] (#1) {}
      },
    } else {
      /tikz/append after command={
        node[%
          fit={(#1-text)},
          inner sep=0pt,
          /litmus/.cd scope={
            every event box/.try={#1},
            event box #1/.try,
          },
        ] (#1) {}
      },
    },
  },
  event/.prefix style={/tikz/anchor=base west},
  % this has to be prefixed so that the 'anchor' of 'going' can
  % take precedence (for all nodes except the first one on the chain)
  init/.style={
    /tikz/name=init-#1,
    /tikz/circle,
    /tikz/minimum size=0.75ex,
    /tikz/inner sep=0,
    /tikz/draw=rf color,
    /tikz/fill=rf color,
    /tikz/node distance=0.75em,
    /tikz/above left=of #1,
    /litmus/.cd scope={
      every init/.try={#1},
      event init-#1/.try,
    },
  },
}

\litmusset{
  init right/.style={
    /litmus/event init-#1/.append style={/tikz/xshift=0.75em, /tikz/right=of #1},
    /litmus/(init-#1) rf (#1)/.append style=/tikz/swap,
  },
  init left/.style={
    /litmus/event init-#1/.append style={/tikz/xshift=-0.75em, /tikz/left=of #1},
  },
  init below/.style={
    /litmus/event init-#1/.append style={/tikz/yshift=-1.25ex, /tikz/below=of #1},
  },
  init above right/.style={
    /litmus/event init-#1/.append style={/tikz/above right=of #1},
    /litmus/(init-#1) rf (#1)/.append style=/tikz/swap,
  },
  init below right/.style={
    /litmus/event init-#1/.append style={/tikz/below /tikz/right=of #1},
    /litmus/(init-#1) rf (#1)/.append style=/tikz/swap,
  },
  init above left/.style={
    /litmus/event init-#1/.append style={/tikz/above left=of #1},
  },
  init below left/.style={
    /litmus/event init-#1/.append style={/tikz/below left=of #1},
    /litmus/(init-#1) rf (#1)/.append style=/tikz/swap,
  },
}

\pgfkeys{
  /litmus/add check exists/.code args={event #1}{%
    \listgadd{\lit@check@exists@list}{#1}%
  },
  /handlers/.change eiid/.style args={to #1}{
    \pgfkeyscurrentpath/.get key parts=\change@temp,
    \change@temp/eiid/.initial={#1},
    /litmus/add check exists/.expand once=\change@tempname,
  },
  /handlers/.change value/.style args={from #1 to #2}{
    \pgfkeyscurrentpath/.get key parts=\change@temp,
    \change@temp/value/.initial={#2},
    \change@temp/value-expected/.initial={#1},
    /litmus/add check exists/.expand once=\change@tempname,
  },
  /handlers/.change addr/.style args={from #1 to #2}{
    \pgfkeyscurrentpath/.get key parts=\change@temp,
    \change@temp/fp addr/.initial={#2},
    \change@temp/fp addr-expected/.initial={#1},
    /litmus/add check exists/.expand once=\change@tempname,
  },
  /handlers/.change offset/.style args={from #1 to #2}{
    \pgfkeyscurrentpath/.get key parts=\change@temp,
    \change@temp/fp offset/.initial={#2},
    \change@temp/fp offset-expected/.initial={#1},
    /litmus/add check exists/.expand once=\change@tempname,
  },
  /handlers/.change size/.style args={from #1 to #2}{
    \pgfkeyscurrentpath/.get key parts=\change@temp,
    \change@temp/fp size/.initial={#2},
    \change@temp/fp size-expected/.initial={#1},
    /litmus/add check exists/.expand once=\change@tempname,
  },
  /handlers/.change footprint/.style args={from #1+#2/#3 to #4+#5/#6}{
    \pgfkeyscurrentpath/.get key parts=\change@temp,
    \change@temp/.change addr=from #1 to #4,
    \change@temp/.change offset=from #2 to #5,
    \change@temp/.change size=from #3 to #6,
  },
  /handlers/.change mem access/.style args={from #1+#2/#3=#4 to #5+#6/#7=#8}{
    \pgfkeyscurrentpath/.get key parts=\change@temp,
    \change@temp/.change addr=from #1 to #5,
    \change@temp/.change offset=from #2 to #6,
    \change@temp/.change size=from #3 to #7,
    \change@temp/.change value=from #4 to #8,
  },
}

\litmusset{
  record exists/.code={\listgadd{\lit@exists@list}{#1}},
  check value/.code 2 args={
    \edef\lit@temp@exval{\pgfkeysifdefined{/litmus/#1-expected}{\pgfkeysvalueof{/litmus/#1-expected}}{#2}}
    \edef\lit@temp@val{#2}
    \ifx\lit@temp@exval\lit@temp@val\else
    \PackageError{litmus-tikz-library}{'#1' does not match the expected value (\lit@temp@exval\space <> \lit@temp@val)}{}
    \fi
  },
  mem event/.style args={#1:#2 #3+#4/#5=#6}{
    % <eiid>:<mem_access> <mem-loc>+<offset>/<size>=<value>
    % e.g. 'a:W x+0/4=1'
    %      'a:Racq x+4/2=5'
    /litmus/record exists={#1},
    /litmus/check value={/litmus/event #1/fp addr}{#3},
    /litmus/check value={/litmus/event #1/fp offset}{#4},
    /litmus/check value={/litmus/event #1/fp size}{#5},
    /litmus/check value={/litmus/event #1/value}{#6},
    /litmus/event contents/.initial={%
      \litmusset{mem access/#2/.try, mem access/.retry={#2}}\,\litmusset{memfp/.expanded={\lit@addr}{\lit@offs}{\lit@size}{\lit@val}}%
    },
    /litmus/event={#1},
    /litmus/event #1/fp addr/.get with default={\lit@addr}{#3},
    /litmus/event #1/fp offset/.get with default={\lit@offs}{#4},
    /litmus/event #1/fp size/.get with default={\lit@size}{#5},
    /litmus/event #1/value/.get with default={\lit@val}{#6},
    /litmus/event contents/.get=\lit@event@contents,
    /tikz/node contents/.expand once=\lit@event@contents,
  },
  mem access/.code={#1},
}

\litmusset{
  boxed events/.default=black!10,
  boxed events/.style={
    /litmus/events box internal/.append style={
      /tikz/rounded corners=2pt,
      /tikz/inner sep=2pt,
      /tikz/fill=#1,
    },
  },
}

\newif\iflit@set@vertical@align@to\lit@set@vertical@align@tofalse
\litmusset{
  horizontal align/.style={
    /tikz/to path={
      (\tikztostart) -- (\tikztotarget |- \tikztostart) \tikztonodes
    },
  },
  set vertical align to/.is global if flag=lit@set@vertical@align@to,
  vertical align to node/.global store in=\lit@vertical@align@to,
  vertical align to/.style={
    /litmus/set vertical align to/.if true=then {
      /litmus/vertical align to node={#1},
      /litmus/set vertical align to=false,
    },
  },
  % after this style is applied all the edges in scope will be vertically
  % aligned with #1 (default: the first node)
  vertical align/.default=\tikztostart,
  vertical align/.style={
    % HACK: clear 'edge distance {0,1}' to locally disable this routing
    /litmus/edge distance {0,1}/.style=,
    /litmus/set vertical align to=true,
    /tikz/to path={
      [/litmus/vertical align to/.expanded={#1}]
      (\tikztostart.south -| \lit@vertical@align@to) -- (\tikztotarget.north -| \lit@vertical@align@to) \tikztonodes
    },
  },
  instruction relations/.style={
    /litmus/vertical align,
    /litmus/.cd scope={
      every instruction relations/.try,
    },
    /tikz/execute at end scope/.value of=/litmus/add to instruction relations \lit@tid,
  },
  /handlers/.add instructions edge/.style={
    \pgfkeyscurrentpath/.get key parts=\lit@key,
    /litmus/add instructions edge/.expand once={\lit@keyname={#1}},
  },
  add instructions edge/.style args={(#1-#2) #3 (#4)=#5}{
    (#1-#2) #3 (#4)/.append style={#5},
    /litmus/add to instruction relations #1/.append={%
      \path (#1-#2) edge[/litmus/.cd scope={#3,#5}] (#4);%
    },
  },
  event relations/.style={
    /litmus/.cd scope={
      every event relations/.try,
    },
    /tikz/execute at end scope/.value of=/litmus/add to event relations,
  },
  /handlers/.add events edge/.style={
    \pgfkeyscurrentpath/.get key parts=\lit@key,
    /litmus/add events edge/.expand once={\lit@keyname={#1}},
  },
  add events edge/.style args={(#1) #2 (#3)=#4}{
    % in most cases it's ok to put #4 in the edge options below
    % (after the #2), but this will not work if there is 'disable edge routing'
    % in side #4, as this key will be evaluated after the routing has
    % already been done. Hence, the following line:
    (#1) #2 (#3)/.append style={#4},
    /litmus/add to event relations/.append={%
      \ifboolexpr{%
        test {\lit@if@init@event{#1}} and%
        not test {\lit@ifnodeexists{#1}}%
      }{% then
        \path node[gobble init/.style args={init-##1}{/litmus/init=##1},gobble init=#1] {} edge[/litmus/.cd scope={#2}] (#3);%
      }{% else
        \path (#1) edge[/litmus/.cd scope={#2}] (#3);%
      }%
    },
  },
}

\def\lit@if@init@event#1{\@lit@if@init@event#1-\par}
\def\@lit@if@init@event#1-#2\par{\ifstrequal{init}{#1}{\@firstoftwo}{\@secondoftwo}}

\litmusset{
  label pos/.initial=0.5,
  label text/.initial=\empty,
  relation/.style={
    /tikz/arrows=->,
    /tikz/thick,
    /tikz/edge node={
      node[
        auto,
        font=\sffamily,
        inner sep=1pt,
        /litmus/.cd scope={
          every label/.try,
          every #1 label/.try,
        },
        pos/.value of=/litmus/label pos,
        node contents/.value of=/litmus/label text,
      ]
    },
    /litmus/.cd scope={
      every relation/.try,
    },
  },
  hide/.style={
    /tikz/overlay, /tikz/to path=, /tikz/opacity=0, /tikz/text opacity=0,
    /tikz/fill opacity=0, /tikz/text height=0, /tikz/text depth=0,
    /tikz/text width=0, /tikz/inner sep=0, /tikz/outer sep=0,
    /tikz/minimum size=0,
  }, % 'to path=' affects 'vertical align' (the first node changes)
}

\litmusset{%
  enable edge routing/.style={
    /litmus/edge routing/.style={
      /utils/ifboolexpe={%
        test {\ifcsdef{lit@\tikztotarget @tid}}%
        and test {\ifcsdef{lit@\tikztostart @tid}}%
        and test {\ifcsdef{lit@\tikztotarget @row}}%
        and test {\ifcsdef{lit@\tikztostart @row}}%
      } then {
        /tikz/evaluate={
          int \x,\y;
          \x = int(\csuse{lit@\tikztotarget @tid}) - int(\csuse{lit@\tikztostart @tid});
          \y = int(\csuse{lit@\tikztotarget @row}) - int(\csuse{lit@\tikztostart @row});
        },
        /litmus/edge distance {\x,\y}/.try,
      },
    },
  },
  disable edge routing/.style={
    /litmus/edge routing/.style=,
  },
  /litmus/edge routing/filter/.is family,
  /litmus/edge routing/.belongs to family=/litmus/edge routing/filter,
  /litmus/disable edge routing/.belongs to family=/litmus/edge routing/filter,
  /litmus/enable edge routing/.belongs to family=/litmus/edge routing/filter,
  /litmus/apply edge routing filter to/.code={%
    \pgfkeys{/pgf/key filters/active families/.install key filter}%
    \pgfqkeysactivatesinglefamilyandfilteroptions{/litmus/edge routing/filter}{/litmus}{#1}%
  },
  /handlers/.disable routing/.style={
    \pgfkeyscurrentpath/disable routing/.style={},
  },
  % Back edges:
  edge distance {-3,-1}/.style={/tikz/out=-160, /tikz/in=-55, /tikz/looseness=0.8, /litmus/label pos=0.9},
  edge distance {-2,-1}/.style={/tikz/out=-160, /tikz/in=-55, /litmus/label pos=0.8},
  edge distance {-1,-4}/.style={/tikz/out=-190, /tikz/in=-145, /tikz/looseness=1},
  edge distance {-1,-3}/.style={/tikz/out=-185, /tikz/in=-145, /tikz/looseness=1.2},
  edge distance {-1,-2}/.style={/tikz/out=-180, /tikz/in=-145, /tikz/looseness=1.5},
  edge distance {-1,-1}/.style={/tikz/out=-160, /tikz/in=-145, /tikz/looseness=2.1, /litmus/label pos=0.8},
  edge distance {0,-1}/.style={/tikz/bend left=60},
  % Loop or events from the same instruction:
  edge distance {0,0}/.style={/tikz/out=180, /tikz/in=180, /tikz/distance=1.5em, /tikz/swap},
  % Immediate successor: for such edges between ioids the 'vertical align'
  % overrides this routing; when such edge exists between eiids you probably
  % want to add 'hide po', '(<eiid1>) <edge> (<eiid2)/.disable routing'
  % and '(<eiid1>) <edge> (<eiid2)/.style={vertical align=<ioid>}' to the
  % litmus diagram.
  edge distance {0,1}/.style={/tikz/bend left=60},
  % Skip (forward) edges:
  edge distance {0,2}/.style={/tikz/bend left=60},
  edge distance {0,3}/.style={/tikz/bend left=60},
  edge distance {0,4}/.style={/tikz/bend left=55},
  edge distance {0,5}/.style={/tikz/bend left=55},
  % Strait horizontal line:
  edge distance {1,0}/.style={
    /tikz/to path={(\tikztostart.east) -- (\tikztotarget.west |- \tikztostart.east) \tikztonodes},
  },
}

% define basic colors
\definecolor{litmusBlack}     {rgb}{0,0,0}             % svgname Black
\definecolor{litmusBrown}     {rgb}{0.647,0.165,0.165} % svgname Brown
\definecolor{litmusRed}       {rgb}{1,0,0}             % svgname Red
\definecolor{litmusOrange}    {rgb}{1,0.648,0}         % svgname Orange
\definecolor{litmusIndigo}    {rgb}{0.294,0.000,0.510} % svgname Indigo
\definecolor{litmusDarkGreen} {rgb}{0.000,0.392,0.000} % svgname DarkGreen

\litmusset{
  /handlers/.litmus relation/.style={
    \pgfkeyscurrentpath/.get key parts=\@lit@key,
    /utils/exec={\expandafter\colorlet\expandafter{\@lit@keyname\space color}{#1}},
    \@lit@key/.default/.expand once=\@lit@keyname,
    \@lit@key/.estyle={
      /litmus/relation={\@lit@keyname},
      /litmus/label text={##1},
      /tikz/color={\@lit@keyname\space color},
      % We run the user defined styles with a special filter that only
      % allowes the '/litmus/{disable|enable} edge routing' keys to be
      % executed, as these keys have to be executed before we do the
      % edge routing and the other keys must be executed after
      /litmus/every \@lit@keyname/.belongs to family=/litmus/edge routing/filter,
      /litmus/(\noexpand\tikztostart) \@lit@keyname\space (\noexpand\tikztotarget)/.belongs to family=/litmus/edge routing/filter,
      /litmus/apply edge routing filter to={
        every \@lit@keyname/.try,
        (\noexpand\tikztostart) \@lit@keyname\space (\noexpand\tikztotarget)/.try,
      },
      % Try all the 'disable routing' options and if none of them work do the routing.
      /litmus/(\noexpand\tikztostart) \@lit@keyname\space (\noexpand\tikztotarget)/disable routing/.try,
      /litmus/(\noexpand\tikztostart)/disable routing/.retry,
      /litmus/(\noexpand\tikztotarget)/disable routing/.retry,
      /litmus/from (\noexpand\tikztostart)/disable routing/.retry,
      /litmus/to (\noexpand\tikztotarget)/disable routing/.retry,
      /litmus/\@lit@keyname/disable routing/.retry,
      /litmus/edge routing/.retry,
      %
      /litmus/.cd scope={
        every \@lit@keyname/.try,
        (\noexpand\tikztostart) \@lit@keyname\space (\noexpand\tikztotarget)/.try,
      },
    },
    /litmus/hide \@lit@keyname/.estyle={\@lit@key/.style={/litmus/hide}},
    /litmus/unhide \@lit@keyname/.estyle={\@lit@key/.litmus relation=#1},
    % Add an inverse edge (not a real edge, just a wrapper that adds
    % \textsuperscript{-1} to the default label)
    \@lit@key^{-1}/.default/.expanded={\expandonce\@lit@keyname\noexpand\textsuperscript{-1}},
    \@lit@key^{-1}/.estyle={\@lit@key={##1}},
  },
  base language/.style={
    % Generated in pp.ml (pp_brief_write_kind):
    /litmus/mem access/W/.code={W},
    % Generated in pp.ml (pp_brief_read_kind):
    /litmus/mem access/R/.code={R},
    /litmus/po/.litmus relation=litmusBlack,
    /litmus/co/.litmus relation=litmusBrown,
    /litmus/rf/.litmus relation=litmusRed,
    /litmus/hide rf/.append style={/litmus/init/.style=/litmus/hide},
    /litmus/rf'/.style 2 args={/litmus/rf={\litmusset{memrf={##1}{##2}}}},
    /litmus/fr/.litmus relation=litmusOrange,
    /litmus/fr'/.style 2 args={/litmus/fr={\litmusset{memfr={##1}{##2}}}},
    /litmus/ctrl/.litmus relation=litmusIndigo,
    /litmus/ctrl+addr/.litmus relation=litmusIndigo,
    /litmus/addr/.litmus relation=litmusIndigo,
    /litmus/data/.litmus relation=litmusIndigo,
    % Edge with multiple labels
    /litmus/multi/.litmus relation=litmusBlack,
    /litmus/multi/separator/.store in=\lit@multi@sep,
    /litmus/multi/separator={,},
    /litmus/append multi label/.code={%
      \pgfkeysgetvalue{/litmus/##1/.@def}{\lit@temp@label@}%
      % Handle inverse edges like 'po^{-1}' (we only look for the ^)
      \def\lit@temp@p####1^####2\lit@term{####1}%
      \edef\lit@temp@label{\expandonce\lit@temp@label{\expandonce\lit@multi@sep}{\noexpand\color{\lit@temp@p##1^\lit@term\space color}\expandonce\lit@temp@label@}}%
    },
    /litmus/multi'/.style={
      /utils/exec={\def\lit@temp@label{\@gobble}},
      /litmus/append multi label/.list={##1},
      /litmus/multi/.expand once=\lit@temp@label,
    },
    %
    /litmus/.cd scope={
      every litmus base language/.try,
    },
  },
  hide edge/.style={/litmus/hide #1},
  hide edges/.style={/litmus/hide edge/.list={#1}},
  unhide edge/.style={/litmus/unhide #1},
  unhide edges/.style={/litmus/unhide edge/.list={#1}},
}

\input{tikzlibrarylitmus.aarch64}
\input{tikzlibrarylitmus.power}
\input{tikzlibrarylitmus.riscv}
\input{tikzlibrarylitmus.x86}

\litmusset{
  state prefix font/.initial=,
  initial state prefix/.initial={Initial~state:\ },
  final state prefix/.initial={Final~state:\ },
  final state allowed prefix/.initial={Allowed:\ },
  final state forbidden prefix/.initial={Forbidden:\ },
  final state result/.initial=unknown,
  final state result/unknown/.style={/litmus/.cd scope={every final state unknown/.try}},
  final state result/allowed/.style={/litmus/.cd scope={every final state allowed/.try}},
  final state result/forbidden/.style={/litmus/.cd scope={every final state forbidden/.try}},
  final state allowed/.style={
    /litmus/final state result=allowed,
    /litmus/final state prefix={\pgfkeysvalueof{/litmus/final state allowed prefix}},
    /utils/if no value={#1} then {} else {
      /litmus/final state={#1},
    },
    /litmus/expected observations=allowed,
  },
  final state forbidden/.style={%
    /litmus/final state result=forbidden,
    /litmus/final state prefix={\pgfkeysvalueof{/litmus/final state forbidden prefix}},
    /utils/if no value={#1} then {} else {
      /litmus/final state={#1},
    },
    /litmus/expected observations=forbidden,
  },
  %
  table header/.code={
    \node[
      name=table header,
      node distance=0,
      inner sep=0,
      outer sep=0,
      align=left,
      text width=\lit@threads@width - (2*\pgfkeysvalueof{/pgf/inner xsep}) + \pgflinewidth,
      /litmus/litmus name/.get=\lit@name,
      /litmus/architecture/.get=\lit@arch,
      node contents={\rlap\lit@name\hfill\llap\lit@arch},
      /litmus/.cd scope={
        every table header/.try,
      },
      #1, % Should be positioning
    ];
  },
  table header/long name/.style={
    node contents={\rlap\lit@name\hfill\llap{\raisebox{2ex}{\lit@arch}}},
  },
  initial state box/.code={
    \node[
      name=initial state box,
      outer sep=0,
      node distance=0,
      node contents={{\pgfkeysvalueof{/litmus/state prefix font}\pgfkeysvalueof{/litmus/initial state prefix}}\pgfkeysvalueof{/litmus/initial state}},
      text width=\lit@threads@width - (2*\pgfkeysvalueof{/pgf/inner xsep}),
      draw,
      /litmus/.cd scope={
        every box/.try,
        every state/.try,
        every initial state/.try,
      },
      #1, % Should be positioning
    ];
  },
  final state box/.code={
    \node[
      name=final state box,
      outer sep=0,
      node distance=0,
      node contents={{\pgfkeysvalueof{/litmus/state prefix font}\pgfkeysvalueof{/litmus/final state prefix}}\pgfkeysvalueof{/litmus/final state}},
      text width=\lit@threads@width - (2*\pgfkeysvalueof{/pgf/inner xsep}),
      draw,
      /litmus/.cd scope={
        every box/.try,
        every state/.try,
        every final state/.try,
      },
      /litmus/final state result/.selected,
      #1, % Should be positioning
    ];
  },
  %   \TODO{change obs to Y,N and - in san serif, try \footnote, add colors to match the tables}
  expected observations/.initial=unknown,
  expected observations/unknown/.style={/litmus/.cd scope={expected observations unknown/.try}},
  expected observations/allowed/.style={/litmus/.cd scope={expected observations allowed/.try}},
  expected observations/forbidden/.style={/litmus/.cd scope={expected observations forbidden/.try}},
  experimental result/.is choice,
  experimental result/observed/.style={
    /tikz/node contents=Y,
    /litmus/.cd scope={
      experimental result/every observed/.try,
    },
  },
  experimental result/not observed/.style={
    /tikz/node contents=N,
    /litmus/.cd scope={
      experimental result/every not observed/.try,
    },
  },
  experimental result/missing/.style={
    /tikz/node contents={--},
    /litmus/.cd scope={
      experimental result/every missing/.try,
    },
  },
  hw observations box/.code={
    \pgfkeysalso{/litmus/hw observations/.get=\lit@obs}%
    \ifdefempty{\lit@obs}{}{% else
      \begin{scope}[%
        /litmus/hw observations/.get=\lit@obs,
        start chain=observations going base right,
        node distance=1pt,
        /litmus/expected observations/.selected,
      ]
        \node[
          name=hw observations prefix,
          outer sep=0,
          node distance=0,
          node contents={HW observations:},
          on chain,
          /litmus/.cd scope={
            every hw observations prefix/.try,
          },
          #1, % Should be positioning
        ];
        \foreach \o/\r in \lit@obs
          \node[
  %           anchor=base west,
  %           at={(hw observations prefix.base east)},
            on chain,
            minimum size=0, inner sep=0, outer sep=0,
            node contents=,
            /litmus/.cd scope={
              every hw observation/.try,
            },
            /utils/ifboolexpr={test {\ifdefstring{\r}{0}}} then {
              /litmus/experimental result=missing,
            } else {
              /utils/ifboolexpr={test {\ifdefstring{\o}{0}}} then {
                /litmus/experimental result=not observed,
              } else {
                /litmus/experimental result=observed,
              },
            },
  %           /litmus/experimental result/.expand once=\s,
          ];
      \end{scope}
    }%
  },
  table construction/.style={
    /litmus/table header={/tikz/above=1pt of threads box, /tikz/anchor=base},
    /litmus/initial state box={/tikz/below=2pt of threads box},
    /litmus/final state box={/tikz/below=of initial state box},
    /litmus/hw observations box={/tikz/anchor=north west,/tikz/at=(final state box.south west)},
  },
  read states file/.code={%
    \begingroup%
      \InputIfFileExists{#1.states.tex}{}{%
        \def\litmusname{??}%
        \def\litmusarch{??}%
        \def\rmemmodel{??}%
        \def\initstate{??}%
        \def\finalstate{??}%
      }%
      \InputIfFileExists{#1.hw.tex}{}{%
        \def\litmusobservations{}%
      }%
      \edef\lit@temp{%
    \endgroup%
        \noexpand\pgfkeysalso{%
          /litmus/litmus name/.initial={\litmusname},%
          /litmus/architecture/.initial={\litmusarch},%
          /litmus/rmem model/.initial={\rmemmodel},%
          /litmus/initial state/.initial={\initstate},%
          /litmus/final state/.initial={\finalstate},%
          /litmus/hw observations/.initial={\litmusobservations},%
        }%
      }\lit@temp%
    \pgfkeysalso{%
      % In most case, the relaxed model indicates the test is forbidden
      % and any other model indicates the test is allowed:
      /litmus/rmem model/.try selected,%
      /litmus/final state allowed/.retry,%
    }%
  },
}
\litmusset{
  litmus table/.style n args={4}{
    /litmus/.cd scope={every litmus table/.try},
    /litmus/litmus name/.initial={#1},
    /litmus/architecture/.initial={#2},
%     /litmus/rmem model/.initial={#??},
    /litmus/initial state/.initial={#3},
    /litmus/final state/.initial={#4},
    /litmus/@litmus table,
    /litmus/hw observations/.initial=,
  },
  @litmus table/.style={
    /tikz/execute at end scope={
      \begin{scope}[/litmus/.cd scope={every table scope/.try}]
        \begin{scope}[on background layer]
          % Fit a node for each assembly line (behind the borders)
          \tikzmath{
            coordinate \@topleft,\@botright;
            \@topleft = (threads-1.north west);
            \@botright = (threads-\chaincount{threads}.north east) - (0pt,\assemrowsep);
            int \@l;
            for \@l in {1,...,\maxassemlines}{
              {%
                \node[%
                  inner sep=0, minimum size=0,
                  yshift=-(\@l - 1) * (\assemrowsep),
                  fit=(\@topleft) (\@botright),
                  node contents=,
                  /litmus/.cd scope={
                    every code line/.try/.expand once=\@l,
                    evaluate={\lit@line@parity = isodd(\@l) ? "odd" : "even";},
                    every \lit@line@parity\space code line/.try/.expand once=\@l,
                    every code line \@l/.try,
                  },
                ];
              };
            };
          }
          % This node fits around all the assembly and thread headers
          \node[
            inner sep=0, outer sep=0,
            /utils/exec={\def\lit@temp@nodes{}},
            evaluate={
              int \c,\t,\tid;
              \c = int(\chaincount{threads});
              for \t in {1,...,\c}{
                \tid = \t - 1;
                print{%
                  \lit@ifnodeexists{thread \tid\space header}{% then
                    \xdef\lit@temp@nodes{\lit@temp@nodes (threads-\t) (thread \tid\space header)}%
                  }{% else
                    \xdef\lit@temp@nodes{\lit@temp@nodes (threads-\t)};
                  }%
                };%
              };
            },
            fit/.expand once=\lit@temp@nodes,
            draw,
            /litmus/.cd scope={
              every box/.try,
              every threads box/.try,
            },
          ] (threads box) {};
          % Draw lines between threads
          \tikzmath{
            int \c,\t;
            \c = int(\chaincount{threads});
            if \c > 1 then {
              for \t in {2,...,\c}{
                % do not remove the "extra" brackets (see \tikzmath 'print')
                {\path[draw, /litmus/.cd scope={every border between threads/.try}] (threads box.north -| threads-\t.west) -- (threads box.south -| threads-\t.west);};
              };
            };
          }
          % Draw a line between thread headers and assembly
          \path[draw, /litmus/.cd scope={every thread headers border/.try}]
            (threads box.west |- threads-1.north) -- (threads box.east |- threads-1.north);
        \end{scope}
        \tikzmath{
          coordinate \diff;
          \diff = (threads box.north east) - (threads box.south west);
          let \lit@threads@width = \diffx;
          let \lit@threads@height = \diffy;
        }
        % Draw the header, initial state and final state
        \litmusset{table construction}
      \end{scope}
    },
  },
}

\litmusset{
  rmem model/relaxed/.style={
    /litmus/final state forbidden,
  },
}

% \litmusset{
%   table shape/.is choice,
%   table shape/going right/.style={},
%   table shape/3/.style={},
%   table shape/4/.style={},
%   table shape=going right,
%
%   first thread below second/.style 2 args={
%     /tikz/evaluate={
%       let \tid = #1;
%       \ts = int(#1 + 1);
%       \below@ts = int(#2 + 1);
%       let \prev@ts = #1;
%     },
%     /litmus/instructions/.append style={
%       /tikz/evaluate if={\lit@tid == \tid} then {
%         below={4ex of threads-\below@ts.south west},
%       },
%       /tikz/evaluate if={\lit@tid == \tid + 1} then {
%         right=of threads-\prev@ts.north east,
%       },
%     },
%     /litmus/@litmus table/.append style={
%       /tikz/execute at end scope={
%         \begin{scope}[/litmus/.cd scope={every table scope/.try}]
%           \begin{scope}[on background layer]
%             \draw (threads-\ts.north west) -- (threads-\ts.north east);
%             \lit@ifnodeexists{thread \tid\space header}{% then
%               \draw (thread \tid\space header.north -| threads-\ts.west) -- (thread \tid\space header.north -| threads-\ts.east);
%             }{}%
%           \end{scope}
%         \end{scope}
%       },
%     },
%   },
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input wrappers
% for all the following macros:
%   #1 - tikz options (optional)
%   #2 - mode ('events', 'assem' or 'full')
%   #3 - .tikz file without the suffix

% We write to this file litmus tests for which diagrams are needed
% Line format: "<context>:<arch>/<test name>"
\def\lit@opt@context{main}
\newwrite\litmusfigs@file
\immediate\openout\litmusfigs@file=\jobname.litmusfigs
% \closeout\litmusfigs@file

% We have to use this 'if' because putting the code inside \IfFileExists
% requires arguments in the tikz options to have extra #'s
\newif\iflit@file@exists

\litmusset{
  missing file/.style={
    draw=red, very thick,
    fill=red!25,
    font=\tiny\bf, align=left,
  },
}

\newcommand{\inputlitmus}[3][]{%
  \immediate\write\litmusfigs@file{\lit@opt@context:#3}%
  \IfFileExists{#3.tikz}{\lit@file@existstrue}{\lit@file@existsfalse}
  \iflit@file@exists%
    \begin{scope}[/litmus/.cd scope={kind={#2},#1}]%
      \input{#3.tikz}
    \end{scope}%
  \else%
    \PackageWarning{litmus-tikz-library}{missing file: #3.tikz}%
    \begin{scope}
      \node[/litmus/missing file] {??missing #3.tikz file??};%
    \end{scope}%
  \fi%
}

\newcommand{\inputlitmuspicture}[3][]{%
  \immediate\write\litmusfigs@file{\lit@opt@context:#3}%
  \IfFileExists{#3.tikz}{\lit@file@existstrue}{\lit@file@existsfalse}
  \iflit@file@exists%
    \begin{tikzpicture}[/litmus/.cd scope={every litmus picture/.try,kind={#2},#1}]%
      \input{#3.tikz}
    \end{tikzpicture}%
  \else%
    \PackageWarning{litmus-tikz-library}{missing file: #3.tikz}%
    \begin{tikzpicture}%
      \node[/litmus/missing file] {??missing #3.tikz file??};%
    \end{tikzpicture}%
  \fi%
}

\newcommand{\inputlitmustable}[3][]{%
  \inputlitmuspicture[%
    every litmus table/.try,%
    read states file={#3},%
    #1,%
    @litmus table,%
  ]{#2}{#3}%
}


==> tikzlibrarylitmus.listings.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                    %
%         rmem executable model                                      %
%                                                                    %
%   Shaked Flur, University of Cambridge                             %
%   Jon French, University of Cambridge                              %
%   Kathryn Gray, University of Cambridge (when this work was done)  %
%   Robert Norton-Wright, University of Cambridge                    %
%   Christopher Pulte, University of Cambridge                       %
%   Susmit Sarkar, University of St Andrews                          %
%   Peter Sewell, University of Cambridge                            %
%                                                                    %
%  This file is copyright 2010-2017 by the authors above.            %
%                                                                    %
%  All rights reserved.                                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% This library should be loaded using '\usetikzlibrary{litmus.listings}'

\RequirePackage{listings}

\litmusset{
  use listing/.default=,
  use listing/.style={
    /litmus/listing options/.initial={#1},
    /utils/exec={%
      \def\assem{\@ifnextchar[{\@assem}{\@assem[]}}%
      \def\lit@internal@assem{\assem}%
    },
  },
}

% NOTE: 'listing options' might include keys like 'basicstyle=\ttfamily',
% therefore, we should not use \edef in the following code
\def\@assem[#1]{%
  \begingroup%
    \litmusset{listing options/.get=\lit@temp}%
  \expandafter\endgroup\expandafter\lstinline\expandafter[\lit@temp,#1]%
}%


==> tikzlibrarylitmus.power.tex <==
\litmusset{
  Power/.style={
    /litmus/listing options/.if defined=then {
      /litmus/listing options/.prefix={language=Power,}
    },
    /litmus/base language,
    % Generated in pp.ml (pp_brief_write_kind):
    /litmus/mem access/WX/.code={W\textsubscript{X}},
    % Generated in pp.ml (pp_brief_read_kind):
    /litmus/mem access/RX/.code={R\textsubscript{X}},
    /litmus/isync/.litmus relation=litmusIndigo,
    /litmus/ctrl+isync/.litmus relation=litmusIndigo,
    /litmus/sync/.litmus relation=litmusDarkGreen,
    /litmus/lwsync/.litmus relation=litmusDarkGreen,
    /litmus/eieio/.litmus relation=litmusDarkGreen,
    /litmus/.cd scope={
      every Power/.try,
    },
  },
}


==> tikzlibrarylitmus.riscv.tex <==
\litmusset{
  RISCV/.style={
    /litmus/listing options/.if defined=then {
      /litmus/listing options/.prefix={language=RISCV,}
    },
    /litmus/base language,
    % Generated in pp.ml (pp_brief_write_kind):
    /litmus/mem access/W.RCpc/.code={W\textsubscript{RCpc}},
    /litmus/mem access/W.RCsc/.code={W\textsubscript{RCsc}},
    /litmus/mem access/W.aqrl/.code={W\textsubscript{aqrl}},
    /litmus/mem access/Wcon/.code={W\textsubscript{con}},
    /litmus/mem access/Wcon.RCpc/.code={W\textsubscript{con.RCpc}},
    /litmus/mem access/Wcon.RCsc/.code={W\textsubscript{con.RCsc}},
    /litmus/mem access/Wcon.aqrl/.code={W\textsubscript{con.aqrl}},
    % Generated in pp.ml (pp_brief_read_kind):
    /litmus/mem access/R.RCpc/.code={R\textsubscript{RCpc}},
    /litmus/mem access/R.RCsc/.code={R\textsubscript{RCsc}},
    /litmus/mem access/R.aqrl/.code={R\textsubscript{aqrl}},
    /litmus/mem access/Rres/.code={R\textsubscript{res}},
    /litmus/mem access/Rres.RCpc/.code={R\textsubscript{res.RCpc}},
    /litmus/mem access/Rres.RCsc/.code={R\textsubscript{res.RCsc}},
    /litmus/mem access/Rres.aqrl/.code={R\textsubscript{res.aqrl}},
    /litmus/fence.i/.litmus relation=litmusIndigo,
    /litmus/ctrl+fence.i/.litmus relation=litmusIndigo,
    /litmus/fence rw rw/.litmus relation=litmusDarkGreen,
      /litmus/fence rw rw/.default={fence rw,rw},
    /litmus/fence rw r/.litmus relation=litmusDarkGreen,
      /litmus/fence rw r/.default={fence rw,r},
    /litmus/fence rw w/.litmus relation=litmusDarkGreen,
      /litmus/fence rw w/.default={fence rw,w},
    /litmus/fence r rw/.litmus relation=litmusDarkGreen,
      /litmus/fence r rw/.default={fence r,rw},
    /litmus/fence r r/.litmus relation=litmusDarkGreen,
      /litmus/fence r r/.default={fence r,r},
    /litmus/fence r w/.litmus relation=litmusDarkGreen,
      /litmus/fence r w/.default={fence r,w},
    /litmus/fence w rw/.litmus relation=litmusDarkGreen,
      /litmus/fence w rw/.default={fence w,rw},
    /litmus/fence w r/.litmus relation=litmusDarkGreen,
      /litmus/fence w r/.default={fence w,r},
    /litmus/fence w w/.litmus relation=litmusDarkGreen,
      /litmus/fence w w/.default={fence w,w},
    /litmus/fence.tso/.litmus relation=litmusDarkGreen,
    /litmus/.cd scope={
      every RISCV/.try,
    },
  },
}


==> tikzlibrarylitmus.x86.tex <==
\litmusset{
  x86/.style={
    /litmus/listing options/.if defined=then {
      /litmus/listing options/.prefix={language=x86,mathescape=false,}
    },
    /litmus/base language,
    % Generated in pp.ml (pp_brief_write_kind):
    /litmus/mem access/Wlck/.code={W\textsubscript{lck}},
    % Generated in pp.ml (pp_brief_read_kind):
    /litmus/mem access/Rlck/.code={R\textsubscript{lck}},
    /litmus/MFENCE/.litmus relation=litmusDarkGreen,
    /litmus/.cd scope={
      every x86/.try,
    },
  },
}

